Caveats on the first-generation da Vinci Research Kit: latent technical constraints and essential calibrations

Telesurgical robotic systems provide a well established form of assistance in the operating theater, with evidence of growing uptake in recent years. Until now, the da Vinci surgical system (Intuitive Surgical Inc, Sunnyvale, California) has been the most widely adopted robot of this kind, with more than 6,700 systems in current clinical use worldwide [1]. To accelerate research on robotic-assisted surgery, the retired first-generation da Vinci robots have been redeployed for research use as "da Vinci Research Kits" (dVRKs), which have been distributed to research institutions around the world to support both training and research in the sector. In the past ten years, a great amount of research on the dVRK has been carried out across a vast range of research topics. During this extensive and distributed process, common technical issues have been identified that are buried deep within the dVRK research and development architecture, and were found to be common among dVRK user feedback, regardless of the breadth and disparity of research directions identified. This paper gathers and analyzes the most significant of these, with a focus on the technical constraints of the first-generation dVRK, which both existing and prospective users should be aware of before embarking onto dVRK-related research. The hope is that this review will aid users in identifying and addressing common limitations of the systems promptly, thus helping to accelerate progress in the field.

==> files/offset_compensation.tex <==
\section{Compensation for Potentiometer offset errors}
%\label{sec:offset_compensation}

%Firstly, in this appendix section, it is assumed that the potentiometer offsets for the last four joints ($b_{P4}$, $b_{P5}$, $b_{P6}$, $b_{P7}$) have been accurately estimated, as previously stated in the Potentiometer calibration section (Sec. \ref{sec:potentiometer}). Secondly, other kinematic errors, such as cable stretching, backlash, or wrong DH parameters are ignored here. Thirdly, 

\add{This appendix focuses on the impact of potentiometer offset errors on the accuracy of end-effector pose estimation through forward kinematics. These errors result in deviations from the actual joint frames ($0$, $1$, $2$, and $3$) into the virtual frames ($\hat{0}$, $\hat{1}$, $\hat{2}$, and $\hat{3}$). It is posited that the accuracy will not be affected by the potentiometer offset error in a certain joint, provided that there exists a constant homogeneous transformation matrix (${}^{\hat{0}}T_0$) from the virtual base frame ($\hat{0}$) to the actual base frame ($0$), so that the virtual joint frame can be realigned to the actual joint frame despite the offset errors in all the preceding joints. The realignment is achieved by applying a new transformation matrix, which is a combination of the constant transformation (${}^{\hat{0}}T_0$), the result of hand-eye calibration (${}^{c}T_{\hat{0}}$) and any virtual transformations, \textit{e.g.} ${}^{\hat{0}}T_{\hat{1}}$.}

% Together, these transformations ensure that the joint frames are properly aligned and any offset errors are compensated for.

%In here, we focus on the accuracy of the end-effector pose estimation for a surgical instrument by using the kinematic data provided by the dVRK. And we posit that the accuracy will not be affected by the potentiometer offset error in a certain joint, provided that: 
% Assuming that researchers are mainly concerned with estimating the end-effector's pose relative to the camera. This pose is not affected by an offset error, as long as:

%\begin{enumerate}
%    \item There exists a constant homogeneous transformation matrix (${}^{\hat{0}}T_0$) from the virtual base frame ($\hat{0}$) to the actual base frame ($0$);
%    \item The constant transformation (${}^{\hat{0}}T_0$), coupled with the result of hand-eye calibration (${}^{c}T_{\hat{0}}$) and any virtual transformations (e.g. ${}^{\hat{0}}T_{\hat{1}}$), leads to realignment between the virtual and the actual joint frame, compensating for all potentiometer offset errors in the preceding joints. 
    % leads to the realignment of a joint's frame, before reaching the end-effector.
%\end{enumerate}

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/appendix.png}
    \caption{This figure illustrates how hand-eye calibration compensates for the offset error in the first potentiometer with the transformation (${}^{c}T_{\hat{0}}$), from the camera frame ($c$) to the virtual base frame ($\hat{0}$). The new hand-eye calibration matrix ${}^{c}T_{\hat{0}}$ post-multiplied by ${}^{\hat{0}}T_{\hat{1}}$ results in the realignment for joint frame 1  ($1 = \hat{1}$), and hence the following joint frames will be aligned if no offset errors exist in the rest of the joints. Hand-eye calibration is capable of compensating for the potentiometer offset errors only when there exists a constant transformation matrix (${}^{\hat{0}}T_{0}$) from the virtual base frame ($\hat{0}$) to the actual base frame ($0$). It is later proved that hand-eye calibration only addresses the offset error in joint 1, but not in joint 2 or 3.}
    \label{fig:pot_app}
\end{figure}

\add{An example of how hand-eye calibration compensates for the offset error in the first joint is shown in Fig. \ref{fig:pot_app}. The goal is to find a constant transformation (${}^{\hat{0}}T_0$), so that after postmultiplying ${}^{\hat{0}}T_{\hat{1}}$ to the new hand-eye calibration matrix (${}^{c}T_{\hat{0}}$), realignment is achieved for joint 1 ($\hat{1} = 1$). After that, all the following joint coordinate frames will be aligned if no potentiometer offset errors exist in the rest of the joints. For the first joint, the following equation is obtained.}

\begin{equation} \label{eq:offset1}
  {}^{\hat{0}}T_0 = {}^{\hat{0}}T_{\hat{1} = 1} ({}^{0}T_{1})^{-1}
\end{equation}

\add{The same logic also applies when the offset errors in both joint 1 and joint 2 are considered:}

\begin{equation} \label{eq:offset12}
  {}^{\hat{0}}T_0 = {}^{\hat{0}}T_{\hat{1}} {}^{\hat{1}}T_{\hat{2} = 2} ({}^{1}T_{2})^{-1}  ({}^{0}T_{1})^{-1}  
\end{equation}

\add{\noindent in which case, realignment is achieved for the second joint frame ($2 = \hat{2}$). Similarly, when the offset errors in all the first three potentiometers are considered:}

\begin{equation} \label{eq:offset123}
  {}^{\hat{0}}T_0 = {}^{\hat{0}}T_{\hat{1}} {}^{\hat{1}}T_{\hat{2}} {}^{\hat{2}}T_{\hat{3}=3} ({}^{2}T_{3})^{-1} ({}^{1}T_{2})^{-1}  ({}^{0}T_{1})^{-1}  
\end{equation}

\add{Next, the analytical solution for ${}^{\hat{0}}T_0$ is found for the above three cases. With the modified DH transformation matrix being:}

\begin{equation*}
\resizebox{0.5\textwidth}{!}{$^{n-1}T_{n} = \begin{bmatrix}
    c(\theta_n) & -s(\theta_n) & 0 & a_{n-1} \\
    s(\theta_n) c(\alpha_{n-1}) & c(\theta_n) c(\alpha_{n-1}) & -s(\alpha_{n-1}) & -d_n s(\alpha_{n-1}) \\
    s(\theta_n) s(\alpha_{n-1}) & c(\theta_n) s(\alpha_{n-1}) & c(\alpha_{n-1}) & d_n c(\alpha_{n-1}) \\
    0 & 0 & 0 & 1
  \end{bmatrix}$}
\end{equation*}

\add{\noindent where $c()$ and $s()$ represent $sin()$ and $cos()$, respectively, and the DH parameters for the dVRK PSMs being:}

\begin{center}
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
 $n$ & $\alpha_{n-1}$ & $a_{n-1}$ & $d_n$ & $\theta_n$ \\ \hline
 1 & $\frac{\pi}{2}$ & 0 & 0 & $q_1 + \frac{\pi}{2}$\\ 
 2 & $-\frac{\pi}{2}$ & 0 & 0 & $q_2 - \frac{\pi}{2}$\\
 3 & $\frac{\pi}{2}$ & 0 & $q_3 - L_{Rcc}$ & 0\\ 
 \hline
\end{tabular}
\end{center}

\add{After solving Eq. \ref{eq:offset1} by substituting in the DH parameters above ($q_1 = j_1$ into ${}^{0}T_{1}$ and $q_1 = j_1 + \Delta_1$ into ${}^{\hat{0}}T_{\hat{1} = 1}$), the following constant transformation is obtained:}

\begin{equation*}
^{\hat{0}}T_{0} = \begin{bmatrix}
    c(\Delta_1) & 0 & -s(\Delta_1) & 0 \\
    0 & 1 & 0 & 0 \\
    s(\Delta_1) & 0 & c(\Delta_1) & 0 \\
    0 & 0 & 0 & 1
  \end{bmatrix}
\end{equation*}

\add{\noindent where $\Delta_1$ is the offset error in the first potentiometer (a constant value). This transformation represents a pure rotation around the y-axis of the actual base frame (0) by $-\Delta_1$.}

\add{Now, assume that $\Delta_1 = 0$ to single out the contribution of the offset error in the second potentiometer to $^{\hat{0}}T_{0}$ and solve Eq. \ref{eq:offset12} (substituting $q_2 = j_2 + \Delta_2$ into ${}^{\hat{1}}T_{\hat{2}}$ and $q_2 = j_2$ into ${}^{1}T_{2}$, the following transformation is obtained:}

\begin{equation*}
\resizebox{0.5\textwidth}{!}{$^{\hat{0}}T_{0} = \begin{bmatrix}
    c(j_1)^2+c(\Delta_2)s(j_1)^2 & s(\Delta_2)s(j_1) & -((-1+c(\Delta_2))c(j_1)s(j_1)) & 0 \\
    -s(\Delta_2)s(j_1) & c(\Delta_2) & c(j_1)s(\Delta_2) & 0 \\
    -((-1+c(\Delta_2))c(j_1)s(j_1)) & -c(j_1)s(\Delta_2) & c(\Delta_2)c(j_1)^2+s(j_1)^2 & 0 \\
    0 & 0 & 0 & 1
  \end{bmatrix}$}
\end{equation*}

\add{\noindent notice that when there exists an offset error in the second potentiometer ($\Delta_2$), $^{\hat{0}}T_{0}$ is not constant because it depends on the value of the first joint ($j_1$).}

\add{Now, assume that $\Delta_1 = 0$, $\Delta_2 = 0$  and solve Eq. \ref{eq:offset123} (substituting $q_3 = j_3 + \Delta_3$ into ${}^{\hat{2}}T_{\hat{3}}$ and $q_3 = j_3$ into ${}^{2}T_{3}$), the following transformation is obtained:}

\begin{equation*}
^{\hat{0}}T_{0} = \begin{bmatrix}
    1 & 0 & 0 & \Delta_3 c(j_2) s(j_1) \\
    0 & 1 & 0 & -\Delta_3s(j_2) \\
    0 & 0 & 1 & - \Delta_3 c(j_1) c(j_2) \\
    0 & 0 & 0 & 1
  \end{bmatrix}
\end{equation*}

\add{Again, note that the offset error in the third potentiometer ($\Delta_3$) induces a non-constant translation between $\hat{0}$ and $0$, which depends on the values of both the first and the second joint ($j_1$ and $j_2$).}

\add{Therefore, it is concluded that a single hand-eye calibration only compensates for the offset error in the first potentiometer ($\Delta_1$) but not for the errors in the second or third potentiometer ($\Delta_2$ and $\Delta_3$). It also implies that to address the potentiometer offset errors in joint 2 and 3, a non-constant hand-eye calibration matrix needs to be updated on the fly.}
